Disturbance Estimation and Rejection for High-Precision Multirotor Position Control

Many multirotor Unmanned Aerial Systems applications have a critical need for precise position control in environments with strong dynamic external disturbances such as wind gusts or ground and wall effects. Moreover, to maximize flight time, small multirotor platforms have to operate within strict constraints on payload and thus computational performance. In this paper, we present the design and experimental comparison of Model Predictive and PID multirotor position controllers augmented with a disturbance estimator to reject strong wind gusts up to 12 m/s and ground effect. For disturbance estimation, we compare Extended and Unscented Kalman filtering. In extensive in- and outdoor flight tests, we evaluate the suitability of the developed control and estimation algorithms to run on a computationally constrained platform. This allows to draw a conclusion on whether potential performance improvements justify the increased computational complexity of MPC for multirotor position control and UKF for disturbance estimation.

==> 05_mpc_control.tex <==
\section{MPC CONTROL FORMULATION}

\subsection{Attitude Dynamics}
\subsection{Optimal Control Problem}

==> abstract.tex <==
\begin{abstract}
	Abstract goes here.
\end{abstract}

==> introduction.tex <==
\section{INTRODUCTION}

